Separator logic and star-free expressions for graphs

We describe two formalisms for defining graph languages, and prove that they are equivalent: 1. Separator logic. This is first-order logic on graphs which is allowed to use the edge relation, and for every $n \in \{0,1,\ldots \}$ a relation of arity $n+2$ which says that "vertex $s$ can be connected to vertex $t$ by a path that avoids vertices $v_1,\ldots,v_n$". 2. Star-free graph expressions. These are expressions that describe graphs with distinguished vertices called ports, and which are built from finite languages via Boolean combinations and the operations on graphs with ports used to construct tree decompositions. Furthermore, we prove a variant of Sch\"utzenberger's theorem (about star-free languages being those recognized by a periodic monoids) for graphs of bounded pathwidth. A corollary is that, given $k$ and a graph language represented by an \mso formula, one can decide if the language can be defined in either of two equivalent formalisms on graphs of pathwidth at most $k$.

==> old-categories.tex <==
\subsection{Categories instead of monoids}
One natural algebraic approach would be to see path decompositions as words (over an alphabet which describes graph operations), and to use homomorphisms from such words into finite monoids. This is almost the approach that we take, but with one minor difference. There is a natural typing relation on path decompositions, namely the numbers of vertices which appear in the leftmost and rightmost bags, respectively. It is natural to assume that path  decompositions are  composed in a way which respects this types; to model this we will use a category structure. 

In our algebraic approach to graphs of pathwidth $k$, we will view path decompositions and their underlying graphs as a category, with objects being numbers $\set{0,1,\ldots,k}$. The idea is that a arrow from object $i$ to object $j$ will describe a path decomposition of width at most $k$ which has $i$ vertices in the first bag and $j$ vertices in the last bag. Composition of such arrows will correspond to concatenation of path decompositions. In the category setting, the role of finite monoids will be played by finite categories, and the role of monoid homomorphisms will be played by functors of categories.  This is only a minor change, and the exact definitions are given in Section~\ref{sec:categories}.



\subsubsection{Categories}
\label{sec:categories}
From the point of view of this paper, the only interest in categories is that they can be seen as mild  generalization of a monoids which allows input and output types for each monoid element. We will not use any  actual category theory. Also, we consider categories with a fixed and finite set of objects $\Oo$.   Recall that a \emph{category} with objects $\Oo$  consists of a set of    \emph{arrows}, with each arrow having designated source and target objects. An arrow with source object $\tau$ and target object $\sigma$ is called an arrow of type $\tau \to \sigma$.  Also a category comes with a composition operation for arrows: an arrow $a$  of type $\tau \to \sigma$ can be composed with a arrow $b$ of type $\sigma \to \rho$, resulting in a arrow $ab$ of type $\tau \to \rho$. Composition of arrows is assumed to be associative, i.e.~$(ab)c = a(bc)$. Finally, we assume that every object $\tau$ comes equipped with distinguished \emph{identity} arrow of type $\tau \to \tau$, with the expected axiom that pre-composing or post-composing with the identity does not change any arrow.


\subsubsection{Languages in categories.}   If $C$ and $D$ are categories with the same objects, then a  \emph{homomorphism}  $\alpha :  C \to D$ is any function $\alpha$ which maps arrows of $C$ to arrows  $D$ so that:  (a) the types of arrows are not changed; (b) composition is preserved; (c) the identity arrows are preserved. In the terminology of category theory, this is a functor that is the identity on objects. A \emph{language} in a category $C$  is defined to be any set of arrows in $C$, such that all arrows in the language have the  same type. We say that a language  in a category $C$ is \emph{recognised} by a homomorphism $\alpha : C \to  D$
     if  membership of an arrow in the language depends only on its image under $\alpha$. A language is called \emph{recognizable} if it is recognized by a homomorphism into a category which is finite in the sense of having finitely many arrows. 

  In a category, the role of letters will be played by some distinguished arrows, and the role of words will be played by arrows generated by the distinguished ones. 
We say that a category is \emph{generated} by  a set of arrows $\Sigma$ if every arrow in the category can be obtained by composing finitely many arrows from $\Sigma$.  
% An important point of departure from the usual theory of regular languages is that we will care about languages in categories that are finitely generated, but not necessarily freely generated, in the sense that there could be two distinct paths that use only generators and yet  describe the same arrow.
 If a category $C$ is finitely generated, then a homomorphism from $C$  into a finite category  can be represented in a finite way: by listing the finite set of arrows of the target category, giving the finite  multiplication table for their composition,  and specifying the values of the functor on the finitely many generators.

 If $\alpha$ and $\beta$ are two homomorphisms with the same domain, then we say that $\alpha$ refines $\beta$ if every arrows $a,b$ satisfy
 \begin{align*}
 \alpha(a) = \alpha(b) \qquad \text{implies} \qquad \beta(a)= \beta(b).
 \end{align*}
 As usual for algebras recognizing languages of finite objects, every language, not necessarily recognizable,   has a canonical recognizing homomorphism.


\begin{theorem}[Syntactic homomorphisms] For every language in a category, there is a homomorphism   which recognizes the language, and which is refined by every other surjective recognizing homomorphism. 
\end{theorem}
\begin{proof}
    A standard proof: we consider two arrows  of same type in the category to be equivalent if there is no path in the category such that replacing one arrow with the other affects membership of the path in $L$. The function which maps an arrow to its equivalence class is the homomorphism from the statement of the lemma.
\end{proof}

The homomorphism from the above theorem is unique, up to isomorphisms on the target algebra, and it is called the \emph{syntactic homomorphism}. A language is recognizable if and only if its syntactic algebra, i.e.~the target algebra of its syntactic homomorphism, is finite.

\subsubsection{Monoids and Green's relations}
\label{sec:greens-relations} Let $A$ be a finite monoid. We use the following definitions, which are based on Green's relations, but with terminology about infixes and prefixes being based on~\cite[Section 1.2]{bojanczyk_recobook}. A \emph{path} in a category is defined to be a sequence of arrows, such that the target object of each arrow in the sequence is equal to the source object of the next arrow. The product of a path is the arrow which  which is the result of composing all arrows in the path; this product does not depend on the order in which arrows from the path are composed. We say that arrow $a$ is a \emph{prefix} of  arrow $b$ if there is a path that begins with arrow $a$ and has product $b$; symmetrically we define \emph{suffixes}. We say that $a$ is an \emph{infix} of $b$ if there is a path which uses arrow $a$ and has product $b$. The prefix, suffix and infix relations are all pre-orders, i.e.~they are transitive and reflexive, but not necessarily anti-symmetric. Two arrows are called \emph{prefix equivalent} if they are prefixes of each other, likewise we define suffix equivalence and infix equivalence. Define an $\Hh$-class to be a nonempty intersection of some prefix class with some suffix class. All arrows in a given $\Hh$-class have the same type, since the  source object is fixed by the prefix class and the target object is fixed by the suffix class.  The following lemma sums up the properties of Green's relations that will be used in our proofs; these are classical results for monoids and the extension to categories is a straightforward exercise. 

\begin{lemma}[Green's Relations Lemma]\label{lem:green}
    Let $J$ be an infix class in a finite category. Then:
    \begin{enumerate}
        \item \label{it:eggbox} If $a \in J$ is a prefix of $b \in J$, then $b$ is a prefix of $a$; likewise for suffixes.
        \item \label{it:h-classes-same-size}  All $\Hh$-classes contained in $J$ have the same size.
        \item \label{it:h-class-with-idempotent}  If an $\Hh$-class contains an idempotent, then it is a group.
    \end{enumerate}
\end{lemma}
\begin{proof}
    The lemma is known to be true for finite monoids, i.e.~finite categories with one object, see~\cite[Lemmas~1.11--1.14]{bojanczyk_recobook}. The more general case of finite categories easily follows from the case of finite monoids, since a finite category  can be viewed as a monoid as follows: the elements of the monoid are the arrows in the category, plus an absorbing  zero element, which represents ill-typed products. In the monoid, if we take the monoid product of two nonzero elements -- which are arrows from the category -- then the value is the product in the category if defined (i.e.~when the target object of the first arrow is the same as  the source object of the second arrow), and otherwise the value is the absorbing zero element. This monoid representation does not affect Green's relations: if $a$ and $b$ arrows from the category, then $a$ is a prefix of $b$ in the category if and only if $a$ is a prefix of $b$ in the monoid; the same holds for the suffix and infix relations.  Since the conclusion of the lemma is true in the monoid, it must also be true in the category.
\end{proof}


 




==> rubbish.tex <==
 
    We can describe properties of contexts using logic, e.g.~separator logic, by associating a model  to each context.  The ports of the context are described using $2k$ constants, with $k$ constants for the left ports and $k$ constants for the right ports. Since ports need not be defined in a context, we use a slightly non-standard version of first-order logic where constants can be undefined; to check if a constant is defined we use the convention that $c=c$ gives a ``no'' answer for constants $c$ that are undefined. Contexts of bounded pathwidth admit  a version of Courcelle's Theorem: if $\varphi$ is a sentence of monadic second-order logic (possibly with modulo counting quantifiers), then for every $k \in \set{1,2,\ldots}$ there is a homomorphism 
    \begin{align*}
    \alpha : \pw_k \to A
    \end{align*}
    into a finite monoid which recognises $\varphi$ on contexts of pathwidth at most $k$. The proof is the same as in Courcelle's Theorem. The situation is more complicated for the  converse of Courcelle's Theorem --  a formal proof of  the converse of Courcelle's Theorem for contexts of  bounded pathwidth would   require a nontrivial reworking of the existing proof for treewidth, see~\cite[Theorem 2.10]{bojanczykDefinabilityEqualsRecognizability2016a},  and we do not do this here\footnote{The issue is that the transductions in~\cite{bojanczykDefinabilityEqualsRecognizability2016a} output tree decompositions, even if the input graphs have bounded pathwidth. This seems necessary, since defining a path decomposition would require imposing something similar to a linear order on the vertices, and this is impossible for  certain simple graphs, e.g.~graphs without edges.}. 

    
    Let $\alpha$ be the homomorphism which maps a context to its port bijection, and let $\beta$ be the reachability. 
    
    \begin{claim}
        Without loss of generality, we can assume that $\alpha(w)$ is idempotent.
    \end{claim}
    \begin{proof}
        It is not hard to see that $\alpha$ is aperiodic, i.e.~for every $w$ there is some idempotent $e$ such that all sufficiently high powers $w^n$ are mapped by $\alpha$ to this idempotent.  Therefore, assuming that the lemma holds for all contexts $w$ such that $\alpha(w)$ is idempotent, we know that for all sufficiently high powers $n$, the image $\beta(w^n)$ is aperiodic. In particular, there are some two consecutive powers $w^n$ and $w^{n+1}$ whose images under $\beta$ are aperiodic.
    \end{proof}
    
    From now on, we assume that $\alpha(w)$ is an idempotent. This means that for persistent ports, their left and right indices are the same. In other words, there is some 
     $I \subseteq \set{1,\ldots,\ell}$ such that for $i \in I$, both the left $i$-th port and the right $i$-th port are non-persistent (in particular, they are different), and for $i \not \in I$, the $i$-th left port and the $i$-th right port are equal (and therefore persistent).


    
    
    Recall the notion of $\Hh$-classes from Section~\ref{sec:greens-relations}: an $\Hh$ class is the intersection of a prefix class with an suffix class. An infix class is called \emph{$\Hh$-trivial} if all of the $\Hh$-classes contained in it have size one. This is the same as saying that some $\Hh$-class contained in it has size one, because all $\Hh$-classes in a given infix class have the same size, by item~\ref{it:h-classes-same-size} of Lemma~\ref{lem:green}. A finite monoid or category is aperiodic if and only if all of its infix classes are $\Hh$-trivial; this is the setting of \schutz's characterization of star-free languages. As we know, for graphs we cannot assume that all infix classes are $\Hh$-trivial. However, the following lemma, which is an important step in our proof, proves $\Hh$-triviality for infix classes which contain an idempotent and a unique bridge (as long as we restrict to port-monotone contexts). For such infix classes, we will be able to use $\Hh$-triviality to get definability using the same ideas as in \schutz's original proof. For the remaining infix classes, we use other ideas: if an infix class does not contain any idempotents, then it is easy to deal with because it cannot repeat too much, while if an infix class does not contain any unique bridges, then contexts from this infix class can be decomposed into parallel compositions of contexts of smaller pathwidth.


    
    
    \begin{lemma}
        For every context 
    \end{lemma}
    
    be the bags in the path decomposition, and suppose that some bag $X_i$ does not intersect a bridge component $U$. The bridge component must be contained in the bags either to the left, or to the right of $X_i$. Without loss of generality, we assume that the bridge is contained in the bags to the right, i.e.
    \begin{align*}
    U \subseteq \bigcup_{j > i} X_i
    \end{align*}
    
    
    suppose that we do find a bag, let $X$ be the vertices in it,  which contains vertices from at most one bridge component. Take a bridge component that is not represented in $X$, and assume by symmetry that this bridge component is contained in bags of the path decomposition that are strictly after $X$. 
    
    We begin with an observation which, while falling short of a proof, will explain the intuitions used later in the proof.  
    As we have observed before,  if context $w$  has a path decomposition without blockades (which is stronger than our assumption that all path decompositions have no blockades), then every prime factor  of $w$ can be decomposed as $xyz$, where $x$ and $z$ are $k$-generators and $y$ has pathwidth strictly smaller than $w$. Therefore, we could use the  induction assumption on smaller pathwidth to  compute  in separator logic the image of every prime factor of  $w$. At this point, one would expect that we can infer the image of $w$ itself, since this image should depend only on the images of its prime factors.  Unfortunately, it is not clear if such a dependency exists.  The problem is that a context can indeed be obtained from its prime factors, but the way to obtain it is by using fusion, and fusion is not a legitimate operation on contexts of given pathwidth, see the discussion in Example~\ref{ex:problems-with-fusion}.  
    
     To work around the problems described in the previous paragraph, we use the following lemma. 
    
     \begin{lemma}\label{lem:persistent-ports}
         Let $w$ be a context of pathwidth $k$, such that every width $k$ path decomposition of $w$ has no blockades. 
     \end{lemma}
     The above lemma finishes the proof of the induction step in the case when $J$ has no blockades, since a formula of separator logic can guess the factorization form the lemma, and find the value for each of the contexts $w_1,\ldots,w_n$ using the induction assumption on more persistent ports. We are left with proving the lemma, which is done in the rest of this section. 
    
    
     We say that a vertex is \emph{persistent} in an interval of a path decomposition if either all bags from the interval contain the vertex, or all bags from the interval do not contain the vertex. A prime factor is called \emph{persistent} in an interval if all non-port vertices from the prime factor are persistent in the interval; otherwise the prime factor is called \emph{active} in the interval. 
     \begin{lemma}\label{lem:active}
         For every context $w$ of pathwidth $k$ there exists a path decomposition, and a partition of its bags into  intervals such that the number of intervals is bounded by a function of $k$ and  such that each interval satisfies:
         \begin{enumerate}
             \item every port of $w$ is inactive in the interval; and 
             \item the interval satisfies one of the two following conditions:
             \begin{enumerate}
                 \item the leftmost and rightmost bags in the interval are the same;
                 \item at most inner component  of $w$  is active in the interval.
             \end{enumerate}
         \end{enumerate} 
     \end{lemma}
    
     Apply the above lemma, resulting in a path decomposition and a family of chosen intervals. Let $I$ be one of these intervals, and let $w_I$ be the corresponding context. By condition 1, every port is inactive in $I$, and therefore if such a port is present in some bag of $I$, then it is a persistent vertex of $w_I$. Therefore, if some port that is not persistent in $w$ is present in $I$, then the corresponding context has strictly more persistent vertices, and thus its image under $\alpha$ must belong to a strict infix of $J$. We are left with the case where the only ports that appear in $I$ are persistent ports. This case, in fact, cannot happen.  
    
         Suppose that $w$ is a context of pathwidth $k$, and that every decomposition of $w$ has no blockades. Apply Lemma~\ref{lem:active}, yielding a path decomposition $P$ with a partition into intervals, which satisfy either (a) or (b). Consider one of these intervals, and the corresponding context, i.e.~the context whose vertices are those that  that appear in some bag from the interval, whose  left ports are the contents of the leftmost bag in the interval, and whose  right ports are the contents of the rightmost bag in the interval. Using the assumption that $P$ has no blockades, we  will show
    
         \begin{claim}
            Let $w$ be a context with a path decomposition that has no blockades. For every interval in this path decomposition  satisfying (a) or (b) as in Lemma~\ref{lem:active},  the corresponding context has strictly more persistent ports than $w$.
         \end{claim}
         \begin{proof}
            Since the path decomposition has no blockades, in every bag of the path decomposition -- except for the first and last one -- there are vertices from at least two connected components. 
    
             Suppose first that the interval has kind (b), which means that at most one prime factor of $w$ is active in the interval. Since there is no blockade, there must be a vertex that appears in some bag from the interval that is not from the active prime factor. Since the vertex is from an persistent prime factor, then it corresponds to an persistent port in the context corresponding to the interval.
    
             Suppose now that the interval has kind (a), which means that the leftmost and rightmost bags in the interval are the same. This means that in the corresponding context, call it $v$, the left and right ports are the same. If the left and right ports are the same, then 
             \begin{align*}
             v = \myunderbrace{v_1 \cdots v_n}{composition of prime factors,\\
             \scriptsize viewed as contexts}
             \end{align*}
         \end{proof}
        
         Apply  Lemma~\ref{lem:active} to a context $w$ whose image under $\alpha$ is in $J$, yielding a path decomposition together with a partition of its bags into intervals. This path decomposition has no blockades, since every path decomposition of $w$ has no blockades. Therefore, we can apply the claim to show that for each of the chosen intervals, the corresponding context has strictly more persistent ports than $w$. The context $w$ itself is a composition of contexts that correspond to intervals in the path decomposition, and $k$-generators which are used to connect these contexts. Summing up, we have shown  that there exists a factorization 
         \begin{align*}
          w = w_1 \cdots w_n,
         \end{align*}
         such that  $n$ is bounded by a function of $k$ and each of the contexts $w_1,\ldots,w_n$  is either a $k$-generator, or  has strictly more persistent ports than $w$. The values under $\alpha$ of the contexts $w_1,\ldots,w_n$ can be computed in separator logic by induction assumption (since there are more persistent ports), or by virtue of having bounded size. Since $n$ is bounded as well, it follows that the decomposition can be guessed, and hence the image of $w$ can also be computed in separator logic. 
    
    \subsubsection{Proof of Lemma~\ref{lem:active}}
    
    
    
        In the proof of this lemma, we say that a number is \emph{bounded} if it is upper bounded by a number that does not depend on $w$ but only on $k$. Using this terminology, we need to find a path decomposition that can be partitioned into a bounded number of intervals, each one satisfying (a) or (b).
          
        The proof of the lemma is in two steps.
     In the first step, we treat contexts with a bounded number of prime factors, and in the second step we treat the general case. 
    
    
    
    \paragraph*{Step 1.}  In the first step, we show that the lemma is true if the context has a bounded number of prime factors. More precisely, we show that if the context has $\ell$ prime factors and pathwidth at most $k$, then there is a path decomposition which has width at most $k$, and which can be partitioned into intervals satisfying (a)or (b) so that the number of intervals is bounded by a function of $k$ and $\ell$.
    
    Consider a context $w$ which has $\ell$ prime factors. The key observation is the following lemma, which comes from .., and which allows us to rearrange bags so that the number of intervals is bounded by a the number of prime factors, and in each interval only one prime factor is active. 
    
    \begin{claim}
        Let $w$ be a context of pathwidth  $k$, and let $X \cup Y$ be a partition of its non-port vertices, such that there is no edge between $X$ and $Y$.  Then there exists a path decomposition of $w$ which has width $k$ and can be partitioned into $\Oo(k)$ intervals, so that in each of the intervals either only $X$ is active, or only $Y$ is active.
    \end{claim}
    
    We apply the above claim to the partition where $X$ is the  non-vertices from the first prime factor, and $Y$ is the remaining non-port vertices. This gives a path decomposition that is split into a bounded number of intervals, such that in each one either (i) only the first prime factor is active, or (ii) only the remaining prime factors are active. For each interval of kind (ii), we reapply the construction, and we keep on doing this until only a single prime factor of the original context is left. 
    
    This completes the first step, where we assumed that the number of prime factors is bounded. Note that in the first step, we only used kind (b) from the conclusion of the lemma. Intervals of kind (a) will appear in the second step.
    
    \paragraph*{Step 2.} We now treat the general case in the lemma. 
    Consider a path decomposition. Define a \emph{phase}  in the path decomposition to be a maximal inclusion-wise interval where all of the ports -- both left and right -- are persistent. The phases partition the bags of the path decomposition into a bounded number of intervals.
    A prime factor of $w$ is called \emph{local} if it is active in at most one phase; otherwise a prime factor is called non-local. The number of non-local prime factors is bounded, because if a factor is non-local then its vertices must be present in the first bag of some phase, and the number of phases and bag sizes are both bounded.
    
    We claim that the path decomposition can be modified so that it has the same underlying context, the same width and number of phases, and every phase can be partitioned into three consecutive intervals, called sub-phases, so that: in the first and third sub-phase only non-local prime factors are active (and therefore the results from Step 1 can be applied to these sub-phases), and the second sub-phase has kind (a) from the statement of the lemma. To see why this claim is true, define the \emph{local width} of a bag to be the number of vertices in the bag whose corresponding prime factor is local. Inside every phase, we can distinguish a bag with maximal local width, and reorder the path decomposition inside this phase so that all local prime factors inside the phase are active just after this distinguished bag. After the reordering, the three sub-phases are:  before the distinguished bag, the sub-phase where the local prime factors are active, and after the distinguished bag. The second sub-phase satisfies condition (a) from the lemma, because it begins and ends with the distinguished bag. As mentioned before, the other two phases can be further subdivided into a bounded number of intervals that satisfy condition (b), thanks to Step 1. 
    
    
 
    
    % We begin with the following simple observation about aperiodic elements in finite monoids.
    % \begin{claim}\label{claim:aperiodic-almost-all-powers}
    %     An element $a$ of a finite  monoid is aperiodic if and only if almost all powers $n\in \set{1,2,\ldots}$ are such that $a^n$ is are aperiodic.
    % \end{claim}
    % \begin{proof}
    %     The left-to-right implication is immediate: if $a$ is aperiodic then all of its powers are aperiodic. Consider now the right-to-left implication.  Since the monoid is finite, there is some $k$ such that
    %     \begin{align}
    %         \label{eq:first-aperiod}
    %     a^n = a^{n+k} \qquad \text{for almost all $n$}.
    %     \end{align}
    %     If $k=1$ then we are done. Otherwise, from the assumption that almost all powers of $a$ are aperiodic, almost all  $p$ satisfy
    %     \begin{align}
    %         \label{eq:second-aperiod}
    %     a^{n} = a^{n+p} \qquad \text{for almost all $n$}
    %     \end{align}
    %     We can choose $p$ so that it is congruent to $1$ modulo $k$, and therefore combining~\eqref{eq:first-aperiod} and~\eqref{eq:second-aperiod} we get the conclusion of the claim.
    % \end{proof}
    % Using the above claim, we can reduce the lemma to a special case which is easier to manage technically.
    % \begin{claim}\label{claim:port-matching-identity}
    %     We can assume without loss of generality that the port matching function is the identity on some subset $I \subseteq \set{1,\ldots,\ell}$.
    % \end{claim}
    % \begin{proof}
    %     Suppose that we have proved the lemma for $w$ which satisfy additionally the assumption from the claim. Using this, we will show that the lemma holds in general. Let $w$ be a context as in the assumption of the lemma, and let 
    %     \begin{align*}
    %     f : \set{1,\ldots,\ell} \to \set{1,\ldots,\ell}
    %     \end{align*}
    %     be its port matching function. The port matching of $w^n$ is equal to $f^n$. As $n$ grows, the domain of $f^n$ gets smaller, and eventually its size  reaches a stable value. Once the stable value has been reached, the domain and co-domain of $f^n$ are the same set, call it  $I \subseteq \set{1,\ldots,\ell}$.  Furthermore, since $w$ is port-monotone, the function $f^n$ is the identity on $I$. Therefore, we can apply the special case that we have assumed in the claim to conclude that for almost all $n$, the image of $w^n$ under the reachability homomorphism is aperiodic. Therefore, thanks to Claim~\ref{claim:aperiodic-almost-all-powers}, also the image of $w$ under the reachability homomorphism is aperiodic. 
    % \end{proof}
    


\begin{align*}
    w = w_1 \cdots w_n
    \end{align*}
    Because of the difficulties 
     by means of fusion of contexts of equal type (in a suitable generalisation for contexts), however the fusion of two contexts of pathwidth $k$ need not have pathwidth $k$, as illustrated in the following picture:
    \begin{center}
        (picture)
    \end{center}
   
     we know tha images of all prime factors of $w$, then we should also know that image of $w$ itself, because $w$ can be constructed using its prime factors using fusion (adapted to contexts in the natural way), and there should be some kind of compositionality principle regarding fusion. Unfortunately, the algebraic setup that we have chosen for pathwidth at most $k$.
   
     the value of a context can be uniquely determined from the values of its prime factors, as expressed in the following statement:
       \begin{itemize}
           \item[($\dagger$)] For every homomorphism 
           \begin{align*}
               \alpha : \pw_k \to A, 
           \end{align*}
           the value $\alpha(w)$ of a context $w \in \pw_k$ depends only on the multiset 
           \begin{align*}
           \set{ \alpha(v) : v \text{ is a prime factor of $w$}}
           \end{align*}
       
       \end{itemize}
       If ($\dagger$) would be true, and furthermore the dependency on the multiset would only need to look at the multiset up to a certain threshold, then we would be done.  Unfortunately, it is not clear why $(\dagger)$ would be true. 
   
   
       \begin{lemma}\label{lem:loop-prime-factor}
           For every $k \in \set{1,2,\ldots}$ there is some $\ell \in \set{1,2,\ldots}$ such that every context $w$ of pathwidth $k$ can be decomposed as 
           \begin{align*}
           w = w_1 \cdots w_{n} 
           \end{align*}
           so that $n \le \ell$ and   each $w_i$ satisfies one of the following:
           \begin{enumerate}
               \item is a $k$-generator; or
               \item is a loop; or
               \item has a unique prime factor.
           \end{enumerate}
       \end{lemma}
   
       The  lemma has a rather long proof, which will be presented in the next section, but for the moment we use the lemma to finish the task at hand, which is  to show that $\alpha$ is definable on $J$ when $J$ has no blockades. Apply Lemma~\ref{lem:loop-prime-factor} to a context $w$ with $\alpha(w) \in J$,  yielding a decomposition into a bounded number of parts, each one satisfying one of the three conditions in the lemma. The parts which are $k$-generators are definable by virtue of having bounded size. For the parts with a unique prime factor, there must  necessarily be a blockade for vacuous reasons, and therefore the value  under $\alpha$ of such parts a strict infix of $J$ (since $J$ has no blockades) and can thus be defined in separator logic thanks to the induction assumption. We are left with the parts which are loops. It is easy to see that for contexts which are loops, fusion is the same as composition, i.e.~if a context $w$ is a loop and $w_1,\ldots,w_n$ are its prime factors, then 
       \begin{align*}
       w = w_1 \cdots w_n.
       \end{align*}
       Furthermore, the above equation is true regardless of the order of $w_1,\ldots,w_n$ in the following sense: for every $\ell$, the  loops of type $\ell \to \ell$ form a commutative monoid. Therefore, if $w$ is a loop context, then ($\dagger$) holds, i.e.~the image $\alpha(w)$ depends only on the image under $\alpha$ of the multiset of prime factors.  Furthermore, if we look at the image of this monoid under the homomorphism $\alpha$, then the image is a commutative and aperiodic monoid, by aperiodicity of $\alpha$. 
   
       
        In this case, it will be more convenient to consider contexts which are looping, in the sense that the left and right ports are the same. 
       \begin{claim}
           Every context of pathwidth at most $k$ can be decomposed as 
           \begin{align*}
           w = w_1 \cdots w_n
           \end{align*}
           where $n \le 2k$ and each of the contexts $w_1,\ldots,w_n$ is either looping or has at most $k+1$ vertices.
       \end{claim}
       \begin{proof}
           We take a path decomposition of $w$, and distinguish the bags which disagree on at least one neighbouring bag with respect to the ports that they contain. The number of 
       \end{proof}
       To prove (*), for every $a \in J$ we need to write a formula which defines contexts that are mapped to some $a$. The following 
       \begin{claim}
           Without loss of generality we 
       \end{claim}
       This implies a weaker property, namely that every context $w$ in with image in $J$, there exists a path decomposition that has no blockades. By Lemma~\ref{lem:blockades}, every prime factor of $w$ can be decomposed as a concatenation $xyz$ of three contexts, such that $x$ and $z$ have constant size and $y$ has smaller pathwidth. For each prime factor, we guess such a decomposition, and use the induction assumption on smaller pathwidth to compute the values under $\alpha$ of the contexts in such a decomposition. This way, we can compute in separator logic the value under $\alpha$ of every prime factor. Finally, the 
       
   \subsubsection{Aperiodic}
   \subsection{Prime factor lemma}
   
   
   \begin{itemize}
       \item[($\dagger$)] For every homomorphism 
       \begin{align*}
           \alpha : \pw_k \to A, 
       \end{align*}
       the value $\alpha(w)$ of a context $w \in \pw_k$ depends only on the multiset 
       \begin{align*}
       \set{ \alpha(v) : v \text{ is a prime factor of $w$}}
       \end{align*}
   
   \end{itemize}
   We would like to like to say that for every homomorphism $\alpha$, the value $\alpha(w)$ depends only on the multiset of values $\alpha(w_1),\ldots,\alpha(w_n)$. This sounds like a rather benign property, but it turns out to be surprisingly problematic in the algebraic setup that we have chosen for pathwidth $k$.
   
   A \emph{loop context} is a context where the  left and right ports are equal, in the sense that every left port is also a right port and vice versa. A context is called a prime loop if it has exactly one prime factor. Every loop context $w$ can be decomposed as 
   \begin{align*}
   w = w_1 \cdots w_n
   \end{align*}
   where $w_1,\ldots,w_n$ are prime loops.
   
   \begin{lemma}
       Let $w$ be a context of pathwidth  $k$, and let $X \cup Y$ be a partition of its non-port vertices, such that there is no edge between $X$ and $Y$.  Then 
       \begin{align*}
       w = w_1 \cdots w_n
       \end{align*} 
       for some $w_1,\ldots,w_n$ of pathwidth $k$, such that $n$ is bounded by a function of $k$, and  for every $i \in \set{1,\ldots,n}$, either every non-port vertex in $w_i$ is from $X$, or every non-port vertex in $w_i$ is from $Y$.
   \end{lemma}
   
   \begin{lemma}
       Let $w$ be context such that every path decomposition of $w$ has no blockades. There exists a factorization 
       \begin{align*}
       w_1 = w_1 \cdots w_\ell
       \end{align*}
       such that $\ell$ is bounded by a function of $k$, and each $w_i$ is either (i) a loop; or (ii) a $k$-generator; or (iii) has strictly smaller non-port width than $w$. 
   \end{lemma}
   Apply the lemma, yielding a path decomposition  together with a decomposition into a bounded number of intervals intervals that satisfy either (a) or (b). Decompose  $w$ as \begin{align*}
   w = w_1 \cdots w_\ell,
   \end{align*}
   so that each context $w_i$ is either a $k$-generator and thus satisfies (ii) from the present lemma, or corresponds to some interval $I$ in  the  path decomposition that satisfies either (a) or (b). If $I$ satisfies (a), then the corresponding context is a loop, i.e.~it satisfies (i).  To finish the proof of the lemma, we will show that if $I$ satisfies (b), then the corresponding context $w_i$ satisfies  (iii). Let $X$ be the vertices of the unique prime factor which is active in the interval $I$.  Since every path decomposition of $w$ contains a blockade, this means that some bag in the interval $I$ must contain a vertex $x$ which does not belong  to $X$.  Since $X$ is the unique prime factor that is active in $I$, it follows that $x$ is present in all bags of $I$, which means that $x$ is a left and right port of the context among $w_1,\ldots,w_\ell$ which corresponds to $I$. Therefore, this context satisfies condition (iii).
   
   so that each of the contexts $w_1,\ldots,w_\ell$ satisfies one of the conditions (a) or (b) from the lemma. If a context satisfies condition (b), then the 
   
   
   Consider now a context $w$, which is mapped by $\alpha$ to $J$. Apply Lemma.. to $w$, yielding a path decomposition divided into a bounded number of intervals. We can view this path decomposition as a factorization
   \begin{align*}
   w = w_1 \cdots w_\ell
   \end{align*}
   such that each $w_i$ corresponds to a distinguished interval in the path decomposition. Suppose that 
   
   \begin{claim}
   
   \end{claim}
   \begin{claim}
       Every phase can be partitioned into a bounded number of intervals, called \emph{sub-phases}, such that 
   \end{claim}
   
   
   A phase can be viewed as context $w$ 
   
   Define a factorization of $P$ to be a partition of its bags so that each block of the partition is an interval. We first partition the bags of $P$ by grouping together the bags which contain the same ports. This partition is a factorization, since for every port, the bags which contain it form an interval. For the same reason, this partition has at most $2k$ blocks. A prime factor is called \emph{local} if there is a exactly one part of the 
   
   We say that a prime factor is \emph{inactive} in an interval if all bags from the interval intersect the prime factor in the same way; otherwise a factor is \emph{active} in the interval. 
   
   \begin{lemma}
       For every $k \in \set{1,2,\ldots}$ there is some $\ell \in \set{1,2,\ldots}$ such that every context $w$ of pathwidth $k$ can be decomposed as 
       \begin{align*}
       w = w_1 \cdots w_{n} 
       \end{align*}
       so that $n \le \ell$ and   each $w_i$ satisfies one of the following:
       \begin{enumerate}
           \item is a $k$-generator; or
           \item is a loop; or
           \item has a unique prime factor.
       \end{enumerate}
   \end{lemma}
   
   \begin{claim}
           
   \end{claim}
   \begin{proof}
   
   
       
       Consider a path decomposition of $w$, of width $k$, and associate to each bag the set of ports (left or right) that are present in the bag. This set can change at most $2k$ times, since there are at most $2k$ ports and the bags which contain a given port form an interval. An interval where the ports that are present 
   \end{proof}
   
   \begin{claim}
       Every loop context $w$ can be decomposed as 
       \begin{align*}
       w = w_1 \cdots w_n
       \end{align*}
       where each $w_i$ has a unique prime factor.
   \end{claim}
   
   
   Consider a loop context. 
   
